AdvPaint: Protecting Images from Inpainting Manipulation via Adversarial Attention Disruption

The outstanding capability of diffusion models in generating high-quality images poses significant threats when misused by adversaries. In particular, we assume malicious adversaries exploiting diffusion models for inpainting tasks, such as replacing a specific region with a celebrity. While existing methods for protecting images from manipulation in diffusion-based generative models have primarily focused on image-to-image and text-to-image tasks, the challenge of preventing unauthorized inpainting has been rarely addressed, often resulting in suboptimal protection performance. To mitigate inpainting abuses, we propose ADVPAINT, a novel defensive framework that generates adversarial perturbations that effectively disrupt the adversary's inpainting tasks. ADVPAINT targets the self- and cross-attention blocks in a target diffusion inpainting model to distract semantic understanding and prompt interactions during image generation. ADVPAINT also employs a two-stage perturbation strategy, dividing the perturbation region based on an enlarged bounding box around the object, enhancing robustness across diverse masks of varying shapes and sizes. Our experimental results demonstrate that ADVPAINT's perturbations are highly effective in disrupting the adversary's inpainting tasks, outperforming existing methods; ADVPAINT attains over a 100-point increase in FID and substantial decreases in precision.

==> alg/attack_algorithm.tex <==

\begin{algorithm}
\caption{\sys}
\begin{algorithmic}[1]
\State \textbf{Input:} Clean image $x$, perturbation $\delta$, mask set $M$, extracted feature $\phi$, optimization steps $N$, step size $\alpha$, perturbation budget $\eta$, total of $L$ layers in U-Net
\State \textbf{Output:} Adversarial example $x'$
\State Initialize $\delta \sim \mathcal{U}(-\eta, \eta)$
\State $x' \gets x + \delta$
\For{mask \textbf{in} $M$}
    \State $m \gets \text{mask}$
    \State $x_0 \gets x \otimes m$
    \State $x'_0 \gets x' \otimes m$
    \For{$i = 0$ \textbf{to} $N-1$}
        \For{$l = 1$ \textbf{to} $L$}
            \vspace{0.5em}
            \State ($q_s^l, k_s^l, v_s^l) \gets (Q_s^l(\phi(x)), K_s^l(\phi(x)), V_s^l(\phi(x)))$
            \vspace{0.5em}
            \State ($q'_s^l, k'_s^l, v'_s^l) \gets (Q_s^l(\phi(x'_i)), K_s^l(\phi(x'_i)), V_s^l(\phi(x'_i)))$
            \vspace{0.5em}
            \State $ q_c^l, q'_c^l \gets Q_c^l(\phi(x)), Q_c^l(\phi(x'_i))$
            \vspace{0.5em}
        \EndFor
        \State $\mathcal{L}_{attn} \gets \sum\limits_{l} \big( \left\| q'_s^l - q_s^l \right\|^2 + \left\| k'_s^l - k_s^l \right\|^2  + \left\| v'_s^l - v_s^l \right\|^2 \big) + \sum\limits_{l} \big( \left\| q'_c^l - q_c^l \right\|^2$ \big)
        \State $\delta \gets \delta + \alpha \cdot \text{sign}(\nabla_{x'_i} \mathcal{L}_{attn})$
        \State $\delta \gets \text{clip}(\delta, -\eta, \eta)$
        \State $x'_{i+1} \gets x_0 + \delta$
    \EndFor
    \State $x' \gets x'_{N-1}$
\EndFor

\end{algorithmic}
\end{algorithm}


==> sec/3_Method.tex <==
\section{Methodology}
\label{sec:method}

% \begin{figure}  
%     \begin{center}
%     \includegraphics[width=0.95\linewidth, trim={5.4cm 5.3cm 5.4cm 4.2cm}, clip]{ICLR 2025 Template/fig/algorithm.pdf}
%     \end{center}
%     \caption{Algorithm of two-stage optimization procedure.}
%    \label{fig:algorithm}
% \end{figure} 

\input{alg/attack_algorithm}



We propose~\sys, a novel defensive framework to protect images from unauthorized inpainting tasks based on LDMs.
% \Skip{~\sys~generates an adversarial perturbation for a given input image, specifically designed to disrupt the adversary's inpainting tasks, thus preventing further manipulation of the image.}
% \WJ{~\sys~generates an adversarial example specifically designed to fool LDM-based inpainting models by disrupting their ability to capture correct attention, thus preventing manipulations on the image.}
% with this perturbation.
%
Section~\ref{sec:att_block} details the structure and role of the attention blocks in LDMs. 
%s
In Section~\ref{sec:att_loss}, we introduce our adversarial objectives for \sys, which simultaneously disrupt cross-attention and self-attention mechanisms. In Section~\ref{sec:optimization}, we describe the optimization strategy, which applies distinct perturbations to regions inside and outside the bounding boxes encompassing target objects, ensuring robustness across various mask shapes.

\begin{wrapfigure}[15]{r}{7cm}
\vspace{-2mm}
    \includegraphics[width=\linewidth, trim={0cm 12cm 15cm 2cm}]{ICLR 2025 Template/fig/denoiser.pdf}
   \caption{Attention mechanism of U-Net denoiser in LDM.}
   \label{fig:framework}
\end{wrapfigure}


% The attention mechanism in the U-net denoiser $\epsilon_\theta$ of an LDM reconstructs an image from the latent vector via a denoising process. As depicted in Figure~\ref{fig:framework}, each attention block -- a sequence of residual, self-attention, and cross-attention blocks -- is repeated after each downsampling and upsampling operation. The self-attention block takes three components: query $q$, key $k$, and value $v$, each of which is a linear transformation of an input image. The cross-attention blocks obtains $k$ and $v$ sourced from external conditioning inputs (\textit{e.g.} prompts). For each layer $l$, $q$ and $k$ are then multiplied to form the attention map $\mathcal{M}$, which is then used to weight $v$, producing the block output $A$:
The attention mechanism in the denoising U-net $\epsilon_\theta$ is augmented to handle conditions $y$ across various modalities.
As depicted in Figure~\ref{fig:framework}, each attention block -- a sequence of residual, self-attention, and cross-attention blocks -- is applied repeatedly. In the self-attention block, the query $q$, key $k$, and value $v$ are computed as linear transformations of intermediate spatial features extracted from the input image $x$.  We denote the intermediate representation of the U-Net at layer $l$ as $\phi_l(x)$.
%
In cross-attention blocks, while $q$ is derived from the intermediate image features like in self-attention, $k$ and $v$ are linearly projected from embeddings of external conditioning inputs $y$ (e.g., prompts). At each layer $l$, $q$ and $k$ form the attention map $\mathcal{M}$, which then weights $v$, producing the output $A$ of that layer:

\begin{equation}
\mathcal{M} = \text{Softmax}\left(\frac{qk^T}{\sqrt{d}}\right), \quad A = \mathcal{M} \cdot v.
\end{equation}

Here, $d$ is the dimension of $q$ and $k$.
%
In this study, we propose a novel optimization method for crafting adversarial perturbations that target both self- and cross-attention blocks. These perturbations are designed to disrupt the model's ability to generate high-dimensional images by undermining the self-attention mechanism while breaking the alignment between prompt tokens and their corresponding spatial positions in the input image by attacking the cross-attention blocks. Accordingly, this adversarial attack using~\sys~thus prevents unauthorized inpainting tasks that leverage LDMs, effectively protecting released images embedded with our perturbations. Moreover, we introduce a method for leveraging masks that cover modified boundary box of an object during adversarial optimization steps, enabling the generation of per-object adversarial perturbations. This approach allows for precise targeting of specific objects within an image, improving the effectiveness of the adversarial perturbations. %Need more precise reasoning and justifcation of leveraging masks here. 


% \begin{comment}
% \subsection{Mask Generation}
% \label{sec:mask generation}
% Unlike image-to-image and text-to-image applications, inpainting models use masks to separate regions to be inpainted from those to be preserved. We observe that applying a single perturbation across the entire image, as done in prior works, is insufficient for protection \WJ{because ...}, as confirmed in Section~\ref{sec:ablation}. 


% \Skip{Therefore, we propose an optimization method that applies distinct perturbations inside and outside a defined boundary. This boundary is determined by expanding the object's bounding box to create a larger mask.}
% \WJ{To overcome this limitation, we propose an optimization method that applies distinct perturbations inside and outside a defined boundary.}
% All masks used in this paper are generated using the Grounded SAM model~\citep{GroundedSAM}, which detects objects and draws their bounding boxes. We then convert these bounding boxes into masks, $m^{bb}$. However, since inpainting masks may vary in size and shape at inference time, often exceeding the bounding box, we
% % do not use $m^{bb}$ as the boundary. Instead, we
% enlarge the bounding box to create a new mask, $m^{BB}$, by increasing its height and width by a factor of a hyperparameter $\rho$, while keeping its center fixed. This expanded mask provides broader coverage and enhances robustness against diverse mask shapes, as demonstrated in Section~\ref{sec:exp1} and~\ref{sec:ablation}. We also generate various masks (e.g., segmentation mask $m^{seg}$) to evaluate our approach against prior methods. For each mask $m$, we use both the mask and its inverse, $1 - m$, to assess performance in both foreground and background inpainting scenarios.
% \end{comment}

\subsection{Adversarial Attack on Attention Blocks}
\label{sec:att_loss}
We propose a novel optimization method for crafting adversarial perturbations that disrupt the functionalities of both self- and cross-attention blocks.
To attack cross-attention blocks, we design an objective function that disturbs the alignment between prompt tokens and their spatial positions in the input image. We aim to maximize the difference between the query $q$ of the clean image $x$ and that of the adversarial example $x+\delta$, thereby disrupting the self-attention mechanism. Given $q = Q(\phi(x))$, where $\phi(\cdot)$ indicates the extracted features from the previous layer immediately before the self- or cross-attention block and $Q(\cdot)$ is the linear projection operator for $q$, we define the adversarial objective $\mathcal{L}_{cross}$ as follows:
\begin{equation}
% \mathcal{L}_{cross} = \max_{\|\delta\|_\infty \leq \eta} \sum\limits_{l} \left\| Q_c^l(\phi(x+\delta)) - Q_c^l(\phi(x)) \right\|^2.
\mathcal{L}_{cross} = \sum\limits_{l} \left\| Q_c^l(\phi(x+\delta)) - Q_c^l(\phi(x)) \right\|^2.
\label{eq:cross-loss}
\end{equation}
Here,  $l$ represents the $l$-th layer of the cross-attention block $c$. By pushing the query $q$ of $x+\delta$ away from that of $x$, this objective interferes the alignment with the key $k$ and value $v$, both of which are derived from the prompt conditions.

We propose another adversarial objective function that specifically targets the self-attention blocks. Unlike $\mathcal{L}_{cross}$, which only attacks $q$ that interacts with external conditioning inputs, this objective targets all input components---$q$, $v$, and $v$---in the self-attention block. This objective function $L_{self}$ in Equation ~\ref{eq:self-loss} is designed to maximize the difference between these three components of $x$ and $x + \delta$:

\begin{equation}
\begin{aligned}
% \mathcal{L}_{self} = \max_{\|\delta\|_\infty \leq \eta} \sum\limits_{l} \bigg(&  \left\| Q_s^l(\phi(x+\delta)) - Q_s^l(\phi(x)) \right\|^2  \\ 
% & + \left\| K_s^l(\phi(x+\delta)) - K_s^l(\phi(x)) \right\|^2  + \left\| V_s^l(\phi(x+\delta)) - V_s^l(\phi(x)) \right\|^2 \bigg).
\mathcal{L}_{self} = \sum\limits_{l} \bigg(&  \left\| Q_s^l(\phi(x+\delta)) - Q_s^l(\phi(x)) \right\|^2  \\ 
& + \left\| K_s^l(\phi(x+\delta)) - K_s^l(\phi(x)) \right\|^2  + \left\| V_s^l(\phi(x+\delta)) - V_s^l(\phi(x)) \right\|^2 \bigg).
\end{aligned}
\label{eq:self-loss}
\end{equation}

Here, $K(\cdot)$ and $V(\cdot)$ are linear projector for $k$ and $v$, respectively, given that $k = K(\phi(x))$ and $v = V(\phi(x))$.
By maximizing the difference across all components, we aim to disrupt the model ability to understand the semantics and spatial structure of the given clean image $x$. 


\subsection{Two-Stage Optimization}
We argue that the adversarial objectives in previous studies~\citep{Photoguard, AdvDM, Mist, CAAT, SDST} are inadequate for protecting images from adversaries' inpainting tasks. Inpainting tasks inherently involve leveraging a mask for a specific target region and then filling the masked area or replacing the background in the unmasked area. However, in this process, the applied mask removes the perturbations embedded in the protected image, rendering them ineffective at tampering with adversaries' inpainting the masked region.

For example, the inpainted ``orange'' in AdvDM (Figure~\ref{fig:1}) exhibits a noisy background in the \textit{unmasked} regions, while the perturbation has no impact on the generated ``orange" object itself. We observed a similar limitation in Figure~\ref{fig:1} "for every prior adversarial works", where the embedded perturbation only undermines inpainting tasks for the unmasked regions in protected images.

To address this limitation, perturbations in the \textit{unmasked} region should influence the generation process in the \textit{masked} area, and vice versa. To achieve this, we apply two different perturbations: one for the \textit{masked} region, disrupting adversaries' background inpainting, and another for the \textit{unmasked} region, disrupting foreground inpainting. By combining these perturbations, we effectively disrupt both foreground and background inpainting tasks.

Specifically, given a target image to protect, \sys first divides the image into two regions---foreground and background--and performs a two-stage optimization to ensure robust protection against masks of varying sizes and shapes.
%
\sys identifies target objects that the adversary may target using Grounded SAM~\citep{GroundedSAM}. To achieve this, \sys leverages a bounding box $m^{bb}$ around the identified objects. This bounding box is then expanded by a factor of $\rho$ to form a new mask, $m$, by increasing its height and width while keeping the center coordinates of $m^{bb}$ intact. Using the two masks, $m$ and $1 - m$, we employ a two-step optimization process to perturb both the masked and unmasked regions using the adversarial objective in Eq~\ref{eq:attn-loss}.

\begin{equation}
% \mathcal{L}_{attn} = \mathcal{L}_{cross} + \mathcal{L}_{self}.
\delta \coloneqq \arg\max_{\|\delta\|_\infty \leq \eta} \mathcal{L}_{attn} =  \arg\max_{\|\delta\|_\infty \leq \eta} \bigg(\mathcal{L}_{cross} + \mathcal{L}_{self}\bigg).
\label{eq:attn-loss}
\end{equation}

Compared to the single-step perturbation used in prior works, where a single perturbation is applied to the entire image, our two-stage strategy offers greater robustness against various mask configurations, as demonstrated in Section~\ref{sec:exp3} and ~\ref{sec:ablation}.


\subsection{Two-Stage Optimization via Attention Loss}
\label{sec:optimization}

% We propose a novel approach of applying different perturbations to the foreground and background regions of a given image, which contributes to significantly disrupting authorized inpainting tasks for that input image.
We propose a novel approach that targets both cross- and self-attention blocks to effectively disrupt unauthorized inpainting tasks, applying distinct perturbations to the foreground and background regions of an image, thereby increasing robustness to masks of varying shapes and sizes.


%
\textbf{Attention loss} We recognize that the objectives in previous studies are inadequate for providing strong protection in inpainting tasks.
Since perturbations are partially concealed by the applied masks, only the perturbations in the \textit{unmasked} regions influence the generation process, distorting only the uncovered parts of the resulting image. For instance, the inpainted `orange' of AdvDM in Figure~\ref{fig:1} exhibits a noisy background in the \textit{unmasked} regions while the perturbation has no impact on the generated `orange' itself.
% This noisy background is also evident in the image-to-image results in Figure~\ref{fig:5}, which display a similar pattern of noise, further confirming that only the \textit{unmasked} regions are affected. 
The same limitation is observed in other methods using previous objectives, where only the \textit{unmasked} regions are affected, allowing the inpainter to perform properly in the \textit{masked} regions. 

We believe that the weakness of previous works for inpainting stems from their objectives--shifting in latent space (Eq~\ref{eq:latent-loss}) or hindering the denoising process (Eq~\ref{eq:noise-loss}, ~\ref{eq:max noise-loss})-- which do not directly focus on the objects in the given image. Inpainting tasks typically revolve around modifying a primary object in an image, either replacing the existing object in foreground inpainting or altering the surrounding environment in background inpainting. However, prior objectives fail to account for the specific components within an image, making them vulnerable to object-focused tasks like inpainting. \JS{~ OR prior works do not consider conditions where masks cover some portions of perturbations?}

To address this challenge, we focus on the roles of the object in inpainting tasks and aim to disturb the core processes related to the object during generation. Specifically, we target the model’s understanding of spatial and semantic information in the self-attention block and its interaction with prompt tokens in the cross-attention block. This method ensures that perturbations in the \textit{unmasked} regions influence the generation in the \textit{masked} regions, applying perturbations to the object for background inpainting and to the background for foreground inpainting. Thus, we propose \textit{attention-loss}, a combined objectve targeting both blocks:

\begin{equation}
\delta \coloneqq \arg\max_{\|\delta\|_\infty \leq \eta} \mathcal{L}_{attn} =  \arg\max_{\|\delta\|_\infty \leq \eta} \mathcal{L}_{cross} + \mathcal{L}_{self}.
\label{eq:attn-loss}
\end{equation}


\textbf{Two-Stage Optimization} 
Although the object in the image plays a key role in inpainting tasks, simply perturbing the object is insufficient for defense against malicious attacks due to one major uncertainty: we cannot predict which masks the inpainting user will employ.
To address this, we divide the image into two regions--foreground and background--and implement a two-stage optimization for robust protection against masks of varying sizes and shapes.
% We observe that applying a single perturbation across the entire image, as proposed in prior works, is insufficient to provide effective protection in inpainting tasks.
% This is because a uniform perturbation fails to account for the different roles that the foreground and background region play in inpainting tasks, where precise object details are critical for inpainting abuses.
%
Specifically, ~\sys~identifies the target region from the background by leveraging a bounding box $m^{bb}$ around the object, using Grounded SAM~\citep{GroundedSAM}. This bounding box is then expanded by a factor of $\rho$ to form a new mask, $m$, by increasing its height and width while maintaining the center coordinates of $m^{bb}$. Using the two masks, $m$ and $1 - m$, we employ a two-step optimization process to perturb both the within-box and outside-box regions. Compared to the single-step perturbation in prior works, where a single perturbation is applied to the entire image, our two-stage strategy provides greater robustness against various masks, as demonstrated in Section~\ref{sec:exp3},~\ref{sec:ablation}.

% To address this limitation, we propose an optimization method that applies distinct perturbations inside and outside a defined boundary. 
% This boundary is determined by our target object, which serves as the adversary's primary focus in inpainting tasks.
% By targeting the object and its surrounding context separately, we significantly improve the effectiveness of adversarial perturbations, thus undermining the adversary's ability to perform successful inpainting.
